How two-way coupling modifies the multiscale preferential sweeping mechanism

For one-way coupled (1WC) flows, Tom & Bragg (J. Fluid Mech., 871, pp. 244-270, 2019) advanced the analysis of Maxey (J. Fluid Mech., 174, pp. 441-465, 1987), which applied to weakly inertial particles, to particles of arbitrary inertia, and the new theoretical result revealed the role that different scales play in the preferential sweeping mechanism that leads to enhanced particle settling in turbulent flows. Monchaux & Dejoan (Phys. Rev. Fluids, 2, 104302, 2017) showed using direct numerical simulations (DNS) that while for low particle loading the effect of two-way coupling (2WC) on the global flow statistics is weak, 2WC enables the particles to drag the fluid in their vicinity down with them, significantly enhancing their settling, and they argued that 2WC suppresses the preferential sweeping mechanism. We explore this further by considering the impact of 2WC on the contribution made by eddies of different sizes on the particle settling. In agreement with Monchaux & Dejoan, we show that even for low loading, 2WC strongly enhances particle settling, and we show how 2WC modifies the contribution from different flow scales. However, contrary to their study, we show that preferential sweeping remains important in 2WC flows. In particular, for both 1WC and 2WC flows, the settling enhancement due to turbulence is dominated by contributions from particles in straining regions of the flow, but for the 2WC case, the particles in these regions also drag the fluid down with them, leading to an enhancement of their settling compared to the 1WC case.

==> Sections/OldTextFigs.tex <==
%
\begin{figure}
	\centering
	\vspace{0mm}
	{\begin{overpic}
			[trim = 0mm 60mm 0mm 50mm,scale=0.4,clip,tics=20]{Figures/JCI/PDF_Q.pdf}
			\put(47,0){$\mathcal{Q}/2\langle\mathcal{S}^2\rangle$}			
	\end{overpic}}
	\caption{DNS results for $\mathcal{P}(\mathcal{Q})$ for different $St$, and for the 1WC and 2WC cases.}
	\label{PDF_Q}
\end{figure}

\begin{figure}
	\centering
	\vspace{0mm}
			\subfloat[]
	{\begin{overpic}
			[trim = 0mm 60mm 0mm 50mm,scale=0.4,clip,tics=20]{Figures/JCI/U_Q_int.pdf}
			\put(120,-5){$St$}			
			\put(43,60){$A(\alpha_1)/u_\eta$, 1WC}
			\put(43,48){$B(\alpha_1)/u_\eta$, 1WC}			
			\put(43,36){$A(\alpha_1)/u_\eta$, 2WC}
			\put(43,24){$B(\alpha_1)/u_\eta$, 2WC}								
	\end{overpic}}
	\subfloat[]
		{\begin{overpic}
			[trim = 0mm 60mm 0mm 50mm,scale=0.4,clip,tics=20]{Figures/JCI/Ratio_plot.pdf}
			\put(120,-5){$St$}			
			\put(100,159){$B(\alpha_1)/A(\alpha_1)$, 1WC}
			\put(100,146){$B(\alpha_1)/A(\alpha_1)$, 2WC}
			\put(100,135){$B(\alpha_2)/A(\alpha_2)$, 1WC}
			\put(100,123){$B(\alpha_2)/A(\alpha_2)$, 2WC}					
	\end{overpic}}
	\caption{DNS results for (a) $A/u_\eta$ and $B/u_\eta$ and (b) $B/A$ as a function of $St$ and for the 1WC and 2WC cases. In the plots, $\alpha_1=0$ and $\alpha_2=4\langle\mathcal{S}^2\rangle$.}
	\label{u_av_Q}
\end{figure}
\FloatBarrier

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -55mm -3mm,
	scale=0.2,clip,tics=20]{Figures/JCI/JCI_SGSVel_StDep_SSpF_Fig01.eps}
\put(48,0.5){\large{$St$}}
\put(-7,20){\rotatebox{90}{\large{$-\langle u_z(\bm{x}^p(t),t)\rangle / u_{\eta}$}}}
\put(15,56.5){\large{1WC}}
\put(15,48.5){\large{2WC}}
	\end{overpic}}
\caption{Normalized settling velocity enhancement for the one-way (1WC) and two-way (2WC) coupled cases shown as a function of $St$.}
\label{Unfilt_SGSVel_StDep}
\end{figure}

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -55mm -3mm,
	scale=0.2,clip,tics=20]{Figures/JCI/JCI_SGSVel_ReDep_SSpF_Fig01.eps}
\put(48,0.5){\large{$Re_{\lambda}$}}
\put(-7,20){\rotatebox{90}{\large{$-\langle u_z(\bm{x}^p(t),t)\rangle / u_{\eta}$}}}
\put(15,56.5){\large{1WC}}
\put(15,48.5){\large{2WC}}
	\end{overpic}}
\caption{Normalized settling velocity enhancement for the one-way (1WC) and two-way (2WC) coupled cases shown as a function of $Re_{\lambda}$.}
\label{Unfilt_SGSVel_ReDep}
\end{figure}

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -85mm -3mm,
	scale=0.195,clip,tics=20]{Figures/JCI/JCI_SGSVel_StDep_SSpF_Fig03.eps}
\put(48,0.5){\large{$\ell_F / \eta$}}
\put(-8,22){\rotatebox{90}{\Large{$ \frac{ \langle u'_{z}(\bm{x}^p(t),t)\rangle } {\langle u_{z}(\bm{x}^p(t),t)\rangle} $}}}
% \put(88,51.85){\large{$St = 0.3$ 1WC}}
% \put(88,47.05){\large{$St = 0.3$ 2WC}}
% \put(88,42.25){\large{$St = 0.5$ 1WC}}
% \put(88,37.45){\large{$St = 0.5$ 2WC}}
% \put(88,32.65){\large{$St = 0.7$ 1WC}}
% \put(88,27.85){\large{$St = 0.7$ 2WC}}
% \put(88,23.05){\large{$St = 1.0$ 1WC} }
% \put(88,18.25){\large{$St = 1.0$ 2WC}}
% \put(88,13.45){\large{$St = 2.0$ 1WC}}
% \put(88,8.65){\large{$St = 2.0$ 2WC}}
	\end{overpic}}
\caption{Ratio of sub-grid settling velocity enhancement to the `full' settling velocity enhancement for the 1WC (1WC - open symbols, dashed line) and 2WC (2WC - closed symbols, solid line) cases shown as a function of the normalized filtering length $\ell_F/\eta$.}
\label{SGS_by_Unfilt_Vel_StDep_ScaleDep}
\end{figure}

\begin{comment}
\textcolor{magenta}{
\begin{itemize}
    \item Should we briefly summarize why computing $\langle {u'}_{z} \rangle (x^{p}(t),t)$ is appropriate to compare with theory \textcolor{green}{???} \textcolor{magenta}{I meant the first paragraph of Section 3.2 `Testing Methodology' in Tom \& Bragg, 2019}
    \item sharp spectral filter
    \item Averaging for 100 turnover times (Rosa 2016; Also Settling velocity of small inertial particles in homogeneous isotropic turbulence from high-resolution DNS, Rosa et al IJMF 2016)
    \end{itemize}}
\end{comment}

\textcolor{magenta}{Another point Maurizio raised was whether we should comment about the saturation of the 1WC/2WC ratios in these plots and if that would help us to infer the scales up to which 2WC has an effect. Would it be reasonable to claim if we can observe saturation on N = 128, St = 0.3 case in  figure \ref{SGSVel_1WC2WC_ratio_StDep_ScaleDep} and N = 256, St = 1 case in  figure \ref{SGSVel_1WC2WC_ratio_ReDep_ScaleDep}?} \textcolor{red}{In one sense our results show no saturation; 2WC appears to be important at all scales since $\langle{u}_z(\bm{x}^p(t),t)\rangle$ is greater for 2WC than for 1WC at all scales. Perhaps the saturation you are referring to is the saturation of their ratios with increasing $\ell_F$? If so, i'm not sure what the significance of that is; it might just be approaching a constant value simply because $\ell_F$ is approaching the largest scales in the flow (and so the saturation is not really significant).}


==> Sections/WritingPointers.tex <==
\begin{comment}

MINOR POINTS
in figures 6 and 7 "A" and "B" seem not very evocative. Can we describe briefly in the caption what they indicate?
sec 4.4 starts at the end of the page

Ok

INTRODUCTION
Summarize importance of particle settling
discuss previous results (Maxey, Wang and Maxey, explanation on pref sweep)
Experiments gave similar results (2wc by default, but very low volume fraction) 
Most of the experiments observed increasing settling velocity, but there are some observations of decreasing settling vel (Nielsen 1993 first observation of loitering). Only with non linear drag and in peculiar situations for DNS (very rare, see Josin's paper)

Most of the studies for 1wc, but reality is 2wc both theory and practical purposes

Recent studies at higher volume fractions (experimental papers) preferential sweeping is also active in 2wc.

2wc DNSs are not that frequent, especially on the settling enhancement

Monchaux relevant enhancement of setting due to 2wc even at low volume fraction, but the fluid statistics stayed the same more or less

Two mechanisms: preferential sweeping and fluid velocity field modified by the particles (sample a different field)

2019 Josin: two contributions to settling, same discussed in experimental papers.
Aim of the paper: how these two mechanisms are modified at different scales





DNS section

Equations of motion, pressure also modified
Exponential integrators for both fluid and particles
mono-disperse particles
nufft for particle feedback
hipstr and nsp validated against each other, plus nufft validation
mean velocity set to zero for all t, meiburg and monchaux pressure mean gradient balances particles weight
physical justification for this, effect of the ground in the atmosphere, zero mass flux. Leave it to Andy?
Filtering methodology - sharp-spectral filter, interpolating the sub-grid velocities and filtered gradients to particle positions
Table of Re and St
Simonin, Horwitz and Mani, numerical issues on 2wc
.05 is the largest dp/eta for our simulations
Artificial periodicity effects, Fr is large, that's fine
We use Fr=1, we focus on the physical mechanism, not specifically to clouds. The mechanism is independnent of the Froude number. Let Andy check this.
Compared our results from our code and Maurizio code and results match very well




Results

Unfiltered first, two-way coupling enhances
in our range settling up with St and Re
how magnitude of enhancement compares 2017PRF, 2006Bosse, 2021Rosa (underestimated enhancement, may be numerical interpolation or computational particles and/or averaging times) enhancement depends on scale separation, different even if Re are relatively similar. Qualitatively same, quant not
fig 3,4 small scales are very effective in 2wc (fluid drag mech)
Despite that (10^3 enhancement) we don't as a large effect compared to that at the small scales (probably small energy of the small scales)
Q results: pref sampl reduces with 2wc so that's not the reason why settling increases. So it should be the fluid drag.
At small scales fluid velocity at part has large energy.


Josin Comments:
This can be attributed to the fluid drag mechanism, where particles drag the surrounding fluid down with them as they fall down under the influence of gravity. The effect of two-way coupling decreases with increasing scale. This could be explained by the effectiveness of particles to pull eddies of different sizes. 

According to Kolmogorovs's 1941 theory, K41 \cite{pope}, the size and energy associated with an eddy increases with increasing scales. Hence the fluid-drag mechanism would be effective at larger scales as they would be more effective in pulling down eddies of comparable energy. Particles can pull eddies down with them, but the larger eddies would be affected less than smaller eddies.

\textcolor{magenta}{Should we mention that 2WC (and even enhancement due to preferential sweeping) is traditionally ignored in weather forecasting models, but the finding in the PRF paper implies that these models might be under predicting settling velocities etc.? Or is it more appropriate in the conclusions section?}

\end{comment}

\begin{comment}

\begin{figure}
\centering
\vspace{0mm}			
	{\begin{overpic}
	[trim = 0mm -25mm -82mm -3mm,
	scale=0.2,clip,tics=20]{Figures/JCI/JCI_EnSpec_StDep_Fig01.eps}
\put(48,2){\large{$\kappa$}}
\put(-5,28){\rotatebox{90}{\large{$E(\kappa)$}}}		
\put(88.5,51.85){\large{$St = 0.3$ 1WC}}
\put(88.5,47.05){\large{$St = 0.3$ 2WC}}
\put(88.5,42.25){\large{$St = 0.5$ 1WC}}
\put(88.5,37.45){\large{$St = 0.5$ 2WC}}
\put(88.5,32.65){\large{$St = 0.7$ 1WC}}
\put(88.5,27.85){\large{$St = 0.7$ 2WC}}
\put(88.5,23.05){\large{$St = 1.0$ 1WC} }
\put(88.5,18.25){\large{$St = 1.0$ 2WC}}
\put(88.5,13.45){\large{$St = 2.0$ 1WC}}
\put(88.5,8.65){\large{$St = 2.0$ 2WC}}
\put(6,10){
\begin{overpic}[trim = 0mm 0mm 0mm 0mm, scale=0.1,clip,tics=20]
{Figures/JCI/JCI_EnSpec_StDep_Fig02.eps}
\end{overpic}
}
	\end{overpic}}
\caption{Ratio of one-way coupled (1WC) sub-grid settling velocity enhancement to that of the two-way coupled (2WC) case shown as a function of the normalized filtering length $\ell_F/\eta$.}
\label{EnSpec_StDep}
\end{figure}

\end{comment}
